Widely Interpretable Semantic Representation: Frameless Meaning Representation for Broader Applicability

This paper presents a novel semantic representation, WISeR, that overcomes challenges for Abstract Meaning Representation (AMR). Despite its strengths, AMR is not easily applied to languages or domains without predefined semantic frames, and its use of numbered arguments results in semantic role labels, which are not directly interpretable and are semantically overloaded for parsers. We examine the numbered arguments of predicates in AMR and convert them to thematic roles that do not require reference to semantic frames. We create a new corpus of 1K English dialogue sentences annotated in both WISeR and AMR. WISeR shows stronger inter-annotator agreement for beginner and experienced annotators, with beginners becoming proficient in WISeR annotation more quickly. Finally, we train a state-of-the-art parser on the AMR 3.0 corpus and a WISeR corpus converted from AMR 3.0. The parser is evaluated on these corpora and our dialogue corpus. The WISeR model exhibits higher accuracy than its AMR counterpart across the board, demonstrating that WISeR is easier for parsers to learn.

==> tex/acknowledgements.tex <==
\section{Acknowledgements}

We gratefully acknowledge the support of the Electronics and Telecommunications Research Institute (ETRI). Any opinions, findings, conclusions, or recommendations expressed in this material are those of the authors and do not necessarily reflect the views of Amazon.

==> tex/discussion.tex <==
\section{Discussion}\label{sec:discussion}

A potential explanation for why the WISeR parser performed better than the AMR parser could be that many WISeR roles are associated with surface level syntax in the object language.
For instance, a \texttt{topic} argument is often introduced with the preposition \textit{about} or \textit{on}, an \texttt{end} is typically introduced by the preposition \textit{to}, \texttt{start} with \textit{from} or \textit{out of} etc.
These cues are obscured when a single \texttt{ARGx} encodes more than one semantic role, or when one semantic role is encoded by more than one \texttt{ARGx}.
However, in WISeR there is a one-to-one correspondence between relations (edge labels), and their semantic functions (thematic roles).
As such, object language cues indicating the appropriate WISeR relation can be found in the data, making classification easier and increasing parser accuracy.

At present, WISeR is similar to AMR without sense disambiguation or numbered arguments.
This has the advantage of being able to introduce predicate concepts for novel predicates on an
\textit{ad hoc} basis.
In future research, we hope to incorporate additional changes to AMR.

%For instance, AMR makes use of PropBank frames such as \texttt{obligate-01} and \texttt{infer-01} to capture deontic and epistemic readings, respectively, for the modal auxiliary \textit{must}.
%At present, WISeR adopts this practice.
%However, treating a single auxiliary as synonymous with one of two distinct predicates based on whether it is interpreted deontically or epistemically obfuscates the fact that the modal force of \textit{must} is always that of necessity.

